Learning from the experts: From expert systems to machine-learned diagnosis models

Expert diagnostic support systems have been extensively studied. The practical applications of these systems in real-world scenarios have been somewhat limited due to well-understood shortcomings, such as lack of extensibility. More recently, machine-learned models for medical diagnosis have gained momentum, since they can learn and generalize patterns found in very large datasets like electronic health records. These models also have shortcomings - in particular, there is no easy way to incorporate prior knowledge from existing literature or experts. In this paper, we present a method to merge both approaches by using expert systems as generative models that create simulated data on which models can be learned. We demonstrate that such a learned model not only preserves the original properties of the expert systems but also addresses some of their limitations. Furthermore, we show how this approach can also be used as the starting point to combine expert knowledge with knowledge extracted from other data sources, such as electronic health records.

==> mimic3.tex <==

\subsection{Flexibility of the ML approach}
Adding new diseases to expert systems require considerable amount of manual curation; More importantly, these expert models require that the diseases have been well-documented through scientific studies.

In this experiment, we show that machine learned models allow us to quickly add new diseases into the system, as long as there are a reasonable number of examples of cases diagnosed with the corresponding diseases. To illustrate this, we used data from electronic hospital records (EHR). Extracting data from EHRs for diagnosis is a well-known practice both in literature and in practice (see \cite{LiuEHRResearch} for an overview of many of those uses, for example). In our case, we used data from the publicly available mimic-iii dataset (see \cite{mimic3}). 

\noindent{\bf Data from mimic-iii}: Mimic-iii provides access to de-identified clinical notes  of 55,000 patients admitted in intensive care units. We restricted to clinical notes written at the time of discharge. Discharge summary consists of textual description of symptoms, physical findings, complications the patient went through and ends with discharge diagnosis. For this experiment, we focused on the sections corresponding to initial symptoms and the discharge diagnosis. We used an in-house entity extraction system to map textual descriptions to medical concepts corresponding to findings from symptom section and diseases from the discharge diagnosis. Each of these concepts have UMLS\cite{bodenreider_umls_2004} concept unique identifier. There can be multiple discharge diagnosis  since the patient being in icu may have experienced additional complications. To reduce the noise, we considered only diseases that have at least 1000 cases, and also removed diseases with low tf-idf (Example: sepsis, a  commonly occurring condition when admitted to hospital for prolonged time.)  
We further processed the disease list for each case and made sure to assign only one disease through this rule of thumb: the disease needs to be in candidate set and other co-occurring diseases are not the ones that are prevalent in mimic-iii. 
This resulted in 7 new diseases that we can now add to our existing expert system. Out of those, 2 diseases already existed in \VDDxSmall, albeit with slightly different names. We processed those to ensure they were added as new examples cases of the existing diseases instead of a new diagnostic. Once those new cases from the EHR were combined with the \VDDxSmall dataset simulated cases,  we trained the CNN model described above using the combined data set. 

%\TODO{train/test split}

The first row in table \ref{tab:accuracy_on_mimic3_testset} presents the performance results when the trained model was evaluated only on the cases for those 7 diseases from the mimic-iii test set \footnote{Note that overall accuracy on a combined test set remains almost unchanged since it is dominated by the test cases generated synthetically}. We can see a significant reduction, especially in top-1 accuracy compared to  Table \ref{tab:noise_robustness}. 

%\geoff{prematurity is an interesting pick, since VDDx is an adult disease KB and prematurity is a neonatal (pediatrics) disease. also subdural hematoma is in VDDx}

To understand if the drop in performance was due to noisy mappings between findings and diseases in mimic-iii (please see data description above), we did the following experiment: we considered only two diseases, prematurity and subdural hemotoma ,  from mimic-iii. These two diseases are quite distinct, and people admitted into ICU with these two diseases often do not have other complications (except for sepsis), and thereby reducing the noise in medical cases 
%\geoff {not sure if this is true, need to rephrase}. 
We re-trained models combining cases from these two diseases with  \VDDxSmall dataset. On this newly trained model with only two additional diseases, top-1 accuracy on just mimic-iii test cases was .99 while the accuracy was unaffected for the combined or simulated only test cases (results are reported in the second row of table\ref{tab:accuracy_on_mimic3_testset}.  This indicates that the performance drop can be attributed to the noisy data set. 

Through this experiment, we have shown as a  proof of concept that it is possible to generalize to new diseases and findings;  We leave the modeling and optimization of the hybrid expert systems with (potentially noisy) cases from electronic health records as part of future work. 
%\geoff {takeaway is that we can learn phenotyping of diseases}




%Interestingly, the performance of the model on the original test set was 0.94 for top-1 recall. This is better than the 0.92 reported when training on expert system generated test cases. We hypothesize that adding more training examples and variability improves the generalization and robustness of the trained model. We also observe a top-1 accuracy of 0.91 when evaluating on a mix of expert generated and EHR test cases.

%While this last result might seem impressive, we do need to understand what is the performance of the trained moddel on the 11 new diseases. Therefore, we test on MIMIC-3 only test set.

\begin{table}
\centering
\begin{tabular}{c c c c}
\toprule
    \textbf{Train set} &\textbf{Test set} & \textbf{Metric} & \textbf{value} \\
     \midrule
     \multirow{2}{*}{\VDDxSmall  + 7 MIMIC-iii diseases} & \multirow{2}{*}{MIMIC-3 test cases 2 diseases} & top-1 accuracy & 0.63\\
     & & top-3 accuracy                          & 0.90\\
        \midrule
    \multirow{2}{*}{\VDDxSmall  + 2 MIMIC-iii diseases} & \multirow{2}{*}{MIMIC-3 test cases from 2 diseases} & top-1 accuracy & 0.99\\
     & & top-3 accuracy                          & 0.99\\
\bottomrule
\end{tabular}
\caption{Top-n Accuracy on EHR-only test cases when training model on a combination of expert simulated data and EHR data.}
\label{tab:accuracy_on_mimic3_testset}
\vspace{-10pt}
\end{table}

%We note that our model does not perform particularly well on these new diseases. However, it is important to keep in mind that we did not optimize our original model or our training data in any particular way. The goal of this experiment is to showcase the flexibility and possibilities of our approach, but we leave the optimization of the hybrid expert + EHR model for future work.


%\TODO{ Approach: Augment vddx data with cases from mimic iii for a few diseases. Evaluate performance on a test set comprising of both vddx + mimic iii test set. Optionally, consider semigran for evaluation}

% Key takeaways:
% \begin{itemize}
% \item Adding mimic iii helped diagnose more diseases rapidly.
% \item Adding mimic iii did not hurt performance on vddx test set
% \end{itemize}


% Of all diseases S in mimic-iii, identify the subset D that has at least support of 1000 diseases. For each $d \in  D$ , count number of times  d occurs either on its own or in S-D. lets call it count(d,d) if count(d,d) > 300, include d for our mlhc and associate all those datapoints that contributed to count(d,d)



% \subsection{Performance on conditions hierarchy}
% \begin{itemize}
% \item Evaluate performance of some hierarchy of diseases
% What is the performance metric when considering a higher label in the hierarchy is correct
% \end{itemize}


check with geoff: fever example in KB, page 11: expert systems resilient to..
conclusion
how did we get so much space reduction: tables?
simulator explanation
first line in abstract






